ZeST: Zero-Shot Material Transfer from a Single Image

We propose ZeST, a method for zero-shot material transfer to an object in the input image given a material exemplar image. ZeST leverages existing diffusion adapters to extract implicit material representation from the exemplar image. This representation is used to transfer the material using pre-trained inpainting diffusion model on the object in the input image using depth estimates as geometry cue and grayscale object shading as illumination cues. The method works on real images without any training resulting a zero-shot approach. Both qualitative and quantitative results on real and synthetic datasets demonstrate that ZeST outputs photorealistic images with transferred materials. We also show the application of ZeST to perform multiple edits and robust material assignment under different illuminations. Project Page: https://ttchengab.github.io/zest

==> figures/tex/ablation_pipeline_component.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/source/ablation_pipeline_component.png}
    \caption{\textbf{Ablation.} Direct Img2Img Pipeline (InstructPix2Pix with IP Adaptor), Our current pipeline without Depth ControlNet.
    } 
    \label{fig:ablation_pipeline_component}
\end{figure}
